The Hadwiger-Nelson problem with two forbidden distances

In 1950 Edward Nelson asked the following simple-sounding question: \emph{How many colors are needed to color the Euclidean plane $\mathbb{E}^2$ such that no two points distance $1$ apart are identically colored?} We say that $1$ is a \emph{forbidden} distance. For many years, we only knew that the answer was $4$, $5$, $6$, or $7$. In a recent breakthrough, de Grey \cite{degrey} proved that at least five colors are necessary. In this paper we consider a related problem in which we require \emph{two} forbidden distances, $1$ and $d$. In other words, for a given positive number $d\neq 1$, how many colors are needed to color the plane such that no two points distance $1$ \underline{or} $d$ apart are assigned the same color? We find several values of $d$, for which the answer to the previous question is at least $5$. These results and graphs may be useful in constructing simpler $5$-chromatic unit distance graphs.

==> fig8inc.tex <==
\coordinate (AA) at ( 4.15, 4.50);
\coordinate (AB) at ( 6.62, 4.50);
\coordinate (AC) at ( 5.38, 8.01);
\coordinate (AD) at ( 2.92, 8.01);
\coordinate (AE) at ( 8.31, 5.34);
\coordinate (AF) at ( 1.23, 7.17);
\coordinate (AG) at ( 7.07, 1.83);
\coordinate (AH) at ( 0.00, 3.66);
\coordinate (AI) at ( 4.15, 0.84);
\coordinate (AJ) at ( 7.07, 7.17);
\coordinate (AK) at ( 0.00, 5.34);
\coordinate (AL) at ( 7.85, 6.33);
\coordinate (AM) at ( 7.85, 2.67);
\coordinate (AN) at ( 8.41, 4.27);
\coordinate (AO) at ( 6.05, 1.22);
\coordinate (AP) at ( 8.31, 3.66);
\coordinate (AQ) at ( 1.23, 1.83);
\coordinate (AR) at (10.77, 5.34);
\coordinate (AS) at ( 3.69, 7.17);
\coordinate (AT) at (10.31, 0.99);
\coordinate (AU) at ( 2.46, 3.66);
\coordinate (AV) at ( 9.54, 7.17);
\coordinate (AW) at ( 2.46, 5.34);
\coordinate (AX) at (12.00, 3.51);
\coordinate (AY) at ( 8.31, 9.00);
\coordinate (AZ) at ( 1.23, 3.51);
\coordinate (BA) at (10.77, 3.66);
\coordinate (BB) at ( 3.69, 1.83);
\coordinate (BC) at (12.00, 5.49);
\coordinate (BD) at ( 4.93, 0.00);
\coordinate (BE) at ( 2.92, 6.33);
\coordinate (BF) at ( 2.92, 2.67);
\coordinate (BG) at ( 8.31, 0.00);
\draw[red] (AA) to (AC);
\draw[red] (AA) to (AD);
\draw[red] (AA) to (AE);
\draw[red] (AA) to (AF);
\draw[red] (AA) to (AG);
\draw[red] (AA) to (AH);
\draw[red] (AA) to (AI);
\draw[red] (AA) to (AJ);
\draw[red] (AA) to (AK);
\draw[red] (AA) to (AL);
\draw[red] (AA) to (AM);
\draw[red] (AA) to (AN);
\draw[red] (AA) to (AO);
\draw[red] (AA) to (AP);
\draw[red] (AA) to (AQ);
\draw[red] (AB) to (AC);
\draw[blue] (AB) to (AD);
\draw[red] (AB) to (AR);
\draw[red] (AB) to (AS);
\draw[blue] (AB) to (AT);
\draw[red] (AB) to (AU);
\draw[red] (AB) to (AV);
\draw[red] (AB) to (AW);
\draw[blue] (AB) to (AX);
\draw[blue] (AB) to (AY);
\draw[blue] (AB) to (AZ);
\draw[red] (AB) to (BA);
\draw[red] (AB) to (BB);
\draw[blue] (AB) to (BC);
\draw[blue] (AB) to (BD);
\draw[red] (AB) to (BE);
\draw[red] (AB) to (BF);
\draw[blue] (AB) to (BG);
\draw[red] (AC) to (AE);
\draw[red] (AC) to (AF);
\draw[red] (AC) to (AV);
\draw[red] (AC) to (AW);
\draw[red] (AD) to (AJ);
\draw[red] (AD) to (AK);
\draw[blue] (AD) to (AY);
\draw[blue] (AD) to (AZ);
\draw[red] (AE) to (AG);
\draw[red] (AE) to (AX);
\draw[red] (AE) to (AY);
\draw[blue] (AE) to (BE);
\draw[red] (AF) to (AH);
\draw[red] (AF) to (AU);
\draw[red] (AF) to (AZ);
\draw[blue] (AF) to (BF);
\draw[blue] (AG) to (AR);
\draw[red] (AG) to (BA);
\draw[red] (AG) to (BF);
\draw[blue] (AH) to (AS);
\draw[red] (AH) to (BB);
\draw[red] (AH) to (BE);
\draw[red] (AI) to (AM);
\draw[blue] (AI) to (AW);
\draw[red] (AI) to (AZ);
\draw[red] (AI) to (BG);
\draw[red] (AJ) to (AP);
\draw[red] (AJ) to (AR);
\draw[blue] (AJ) to (BA);
\draw[red] (AJ) to (BE);
\draw[red] (AK) to (AQ);
\draw[red] (AK) to (AS);
\draw[blue] (AK) to (BB);
\draw[red] (AK) to (BF);
\draw[red] (AL) to (AM);
\draw[red] (AL) to (AS);
\draw[blue] (AL) to (AW);
\draw[red] (AL) to (BA);
\draw[red] (AL) to (BC);
\draw[red] (AM) to (AR);
\draw[blue] (AM) to (AU);
\draw[blue] (AM) to (AV);
\draw[red] (AM) to (AX);
\draw[red] (AM) to (BB);
\draw[red] (AM) to (BD);
\draw[red] (AN) to (AO);
\draw[red] (AN) to (AT);
\draw[blue] (AN) to (AY);
\draw[blue] (AN) to (BB);
\draw[red] (AO) to (AT);
\draw[blue] (AO) to (AZ);
\draw[blue] (AO) to (BA);
\draw[red] (AP) to (AV);
\draw[red] (AP) to (BC);
\draw[blue] (AP) to (BF);
\draw[red] (AP) to (BG);
\draw[red] (AQ) to (AW);
\draw[red] (AQ) to (BD);
\draw[blue] (AQ) to (BE);
\draw[red] (AS) to (AU);
\draw[blue] (AT) to (BC);
\draw[blue] (AT) to (BD);
\draw[red] (AV) to (BA);
\draw[red] (AW) to (BB);
\draw[blue] (AX) to (BG);
\draw[blue] (AY) to (BC);
\draw[blue] (AZ) to (BD);
\draw[red] (BE) to (BF);
\node[state,fill=cyan] at (AA) {\textbf{A}};
\node[state,fill=cyan] at (AB) {\textbf{B}};
\node[state,fill=yellow] at (AC) {\textbf{1}};
\node[state,fill=yellow] at (AD) {\textbf{2}};
\node[state,fill=yellow] at (AE) {\textbf{3}};
\node[state,fill=yellow] at (AF) {\textbf{4}};
\node[state,fill=yellow] at (AG) {\textbf{5}};
\node[state,fill=yellow] at (AH) {\textbf{6}};
\node[state,fill=yellow] at (AI) {\textbf{7}};
\node[state,fill=yellow] at (AJ) {\textbf{8}};
\node[state,fill=yellow] at (AK) {\textbf{9}};
\node[state,fill=yellow] at (AL) {\textbf{10}};
\node[state,fill=yellow] at (AM) {\textbf{11}};
\node[state,fill=yellow] at (AN) {\textbf{12}};
\node[state,fill=yellow] at (AO) {\textbf{13}};
\node[state,fill=yellow] at (AP) {\textbf{14}};
\node[state,fill=yellow] at (AQ) {\textbf{15}};
\node[state,fill=yellow] at (AR) {\textbf{16}};
\node[state,fill=yellow] at (AS) {\textbf{17}};
\node[state,fill=yellow] at (AT) {\textbf{18}};
\node[state,fill=yellow] at (AU) {\textbf{19}};
\node[state,fill=yellow] at (AV) {\textbf{20}};
\node[state,fill=yellow] at (AW) {\textbf{21}};
\node[state,fill=yellow] at (AX) {\textbf{22}};
\node[state,fill=yellow] at (AY) {\textbf{23}};
\node[state,fill=yellow] at (AZ) {\textbf{24}};
\node[state,fill=yellow] at (BA) {\textbf{25}};
\node[state,fill=yellow] at (BB) {\textbf{26}};
\node[state,fill=yellow] at (BC) {\textbf{27}};
\node[state,fill=yellow] at (BD) {\textbf{28}};
\node[state,fill=yellow] at (BE) {\textbf{29}};
\node[state,fill=yellow] at (BF) {\textbf{30}};
\node[state,fill=yellow] at (BG) {\textbf{31}};

